Quantum hardware calculations of periodic systems with partition-measurement symmetry verification: simplified models of hydrogen chain and iron crystals

Running quantum algorithms on real hardware is essential for understanding their strengths and limitations, especially in the noisy intermediate scale quantum (NISQ) era. Herein we focus on the practical aspect of quantum computational calculations of solid-state crystalline materials based on theory developed in our group by using real quantum hardware with a novel noise mitigation technique referred to as partition-measurement symmetry verification, which performs post-selection of shot counts based on $Z_{2}$ and $U_{1}$ symmetry verification. We select two periodic systems with different level of complexity for these calculations. One of them is the distorted hydrogen chain as an example of very simple systems, and the other one is iron crystal in the BCC and FCC phases as it is considered to be inaccessible by using classical computational wavefunction methods. The ground state energies are evaluated based on the translational quantum subspace expansion (TransQSE) method for the hydrogen chain, and periodic boundary condition adapted VQE for our iron models. By applying these techniques for the simplest 2 qubit iron model systems, the correlation energies obtained by the hardware calculations agree with those of the state-vector simulations within $\sim$5 kJ/mol. Although the quantum computational resources used for those experiments are still limited, the techniques applied to obtain our simplified models will be applicable in essentially the same manner to more complicated cases as quantum hardware matures.

==> iron_mo_bcc.tex <==
\begin{table}
    \small
    \centering
    \caption{
        UHF crystal orbital energies
        $\varepsilon_{k_{p},p,\omega}$
        and its occupation number for the BCC structure
        calculated with $[2~1~1]$ k-points.
        $(k_{p}, p, \omega)$ are indices for
        (k-point, MO, spin).
    }
    \label{tab:iron_mo_bcc}
    \begin{tabular}{crc|crc}
        \hline
        $(k_{p}, p, \omega)$ & $\varepsilon_{k_{p},p,\omega}$ / Ha & Occupation &
        $(k_{p}, p, \omega)$ & $\varepsilon_{k_{p},p,\omega}$ / Ha & Occupation
        \\
        \hline
        $( 0, 0, 0)$ & $ -3.3983$ &  1 &  $( 1, 0, 0)$ & $ -3.3945$ &  1 \\
        $( 0, 1, 0)$ & $ -2.0343$ &  1 &  $( 1, 1, 0)$ & $ -2.0339$ &  1 \\
        $( 0, 2, 0)$ & $ -1.9857$ &  1 &  $( 1, 2, 0)$ & $ -2.0108$ &  1 \\
        $( 0, 3, 0)$ & $ -1.9757$ &  1 &  $( 1, 3, 0)$ & $ -1.9935$ &  1 \\
        $( 0, 4, 0)$ & $  0.1709$ &  1 &  $( 1, 4, 0)$ & $  0.1902$ &  1 \\
        $( 0, 5, 0)$ & $  0.2531$ &  1 &  $( 1, 5, 0)$ & $  0.2426$ &  1 \\
        $( 0, 6, 0)$ & $  0.2548$ &  1 &  $( 1, 6, 0)$ & $  0.2619$ &  1 \\
        $( 0, 7, 0)$ & $  0.2895$ &  1 &  $( 1, 7, 0)$ & $  0.2781$ &  1 \\
        $( 0, 8, 0)$ & $  0.3533$ &  1 &  $( 1, 8, 0)$ & $  0.9708$ &  0 \\
        $( 0, 9, 0)$ & $  0.4998$ &  1 &  $( 1, 9, 0)$ & $  1.2467$ &  0 \\
        $( 0,10, 0)$ & $  2.0892$ &  0 &  $( 1,10, 0)$ & $  1.8842$ &  0 \\
        $( 0,11, 0)$ & $  2.1052$ &  0 &  $( 1,11, 0)$ & $  2.0856$ &  0 \\
        $( 0,12, 0)$ & $  2.2332$ &  0 &  $( 1,12, 0)$ & $  2.5263$ &  0 \\
        $( 0,13, 0)$ & $  2.2435$ &  0 &  $( 1,13, 0)$ & $  3.3282$ &  0 \\
        $( 0,14, 0)$ & $  2.2506$ &  0 &  $( 1,14, 0)$ & $  6.9834$ &  0 \\
        \hline
        $( 0, 0, 1)$ & $ -3.2018$ &  1 &  $( 1, 0, 1)$ & $ -3.1975$ &  1 \\
        $( 0, 1, 1)$ & $ -1.7918$ &  1 &  $( 1, 1, 1)$ & $ -1.8181$ &  1 \\
        $( 0, 2, 1)$ & $ -1.7765$ &  1 &  $( 1, 2, 1)$ & $ -1.7944$ &  1 \\
        $( 0, 3, 1)$ & $ -1.7227$ &  1 &  $( 1, 3, 1)$ & $ -1.7224$ &  1 \\
        $( 0, 4, 1)$ & $  0.1844$ &  1 &  $( 1, 4, 1)$ & $  0.2622$ &  1 \\
        $( 0, 5, 1)$ & $  0.3542$ &  1 &  $( 1, 5, 1)$ & $  0.3016$ &  1 \\
        $( 0, 6, 1)$ & $  0.4409$ &  1 &  $( 1, 6, 1)$ & $  1.0559$ &  0 \\
        $( 0, 7, 1)$ & $  0.5669$ &  1 &  $( 1, 7, 1)$ & $  1.2492$ &  0 \\
        $( 0, 8, 1)$ & $  1.2398$ &  0 &  $( 1, 8, 1)$ & $  1.2609$ &  0 \\
        $( 0, 9, 1)$ & $  1.2434$ &  0 &  $( 1, 9, 1)$ & $  1.3124$ &  0 \\
        $( 0,10, 1)$ & $  2.1964$ &  0 &  $( 1,10, 1)$ & $  1.9106$ &  0 \\
        $( 0,11, 1)$ & $  2.2156$ &  0 &  $( 1,11, 1)$ & $  2.2105$ &  0 \\
        $( 0,12, 1)$ & $  2.2645$ &  0 &  $( 1,12, 1)$ & $  2.6535$ &  0 \\
        $( 0,13, 1)$ & $  2.2790$ &  0 &  $( 1,13, 1)$ & $  3.3528$ &  0 \\
        $( 0,14, 1)$ & $  2.2989$ &  0 &  $( 1,14, 1)$ & $  7.0283$ &  0 \\
        \hline
    \end{tabular}
\end{table}


==> iron_mo_fcc.tex <==
\begin{table}
    \small
    \centering
    \caption{
        UHF crystal orbital energies
        $\varepsilon_{k_{p},p,\omega}$
        and its occupation number for the FCC structure
        calculated with $[2~1~1]$ k-points.
        $(k_{p}, p, \omega)$ are indices for
        (k-point, MO, spin).
    }
    \label{tab:iron_mo_fcc}
    \begin{tabular}{crc|crc}
        \hline
        $(k_{p}, p, \omega)$ & $\varepsilon_{k_{p},p,\omega}$ / Ha & Occupation &
        $(k_{p}, p, \omega)$ & $\varepsilon_{k_{p},p,\omega}$ / Ha & Occupation
        \\
        \hline
        $( 0, 0, 0)$ & $ -3.4252$ &  1 &  $( 1, 0, 0)$ & $ -3.4225$ &  1 \\
        $( 0, 1, 0)$ & $ -2.0541$ &  1 &  $( 1, 1, 0)$ & $ -2.0654$ &  1 \\
        $( 0, 2, 0)$ & $ -2.0458$ &  1 &  $( 1, 2, 0)$ & $ -2.0557$ &  1 \\
        $( 0, 3, 0)$ & $ -1.9852$ &  1 &  $( 1, 3, 0)$ & $ -1.9989$ &  1 \\
        $( 0, 4, 0)$ & $  0.1436$ &  1 &  $( 1, 4, 0)$ & $  0.1832$ &  1 \\
        $( 0, 5, 0)$ & $  0.1998$ &  1 &  $( 1, 5, 0)$ & $  0.2052$ &  1 \\
        $( 0, 6, 0)$ & $  0.2394$ &  1 &  $( 1, 6, 0)$ & $  0.2181$ &  1 \\
        $( 0, 7, 0)$ & $  0.2664$ &  1 &  $( 1, 7, 0)$ & $  0.2768$ &  1 \\
        $( 0, 8, 0)$ & $  0.3262$ &  1 &  $( 1, 8, 0)$ & $  0.8942$ &  0 \\
        $( 0, 9, 0)$ & $  0.5021$ &  1 &  $( 1, 9, 0)$ & $  1.1734$ &  0 \\
        $( 0,10, 0)$ & $  2.0216$ &  0 &  $( 1,10, 0)$ & $  1.8988$ &  0 \\
        $( 0,11, 0)$ & $  2.0515$ &  0 &  $( 1,11, 0)$ & $  1.9154$ &  0 \\
        $( 0,12, 0)$ & $  2.0675$ &  0 &  $( 1,12, 0)$ & $  2.7694$ &  0 \\
        $( 0,13, 0)$ & $  2.4434$ &  0 &  $( 1,13, 0)$ & $  2.8108$ &  0 \\
        $( 0,14, 0)$ & $  2.4509$ &  0 &  $( 1,14, 0)$ & $  3.7054$ &  0 \\
        \hline
        $( 0, 0, 1)$ & $ -3.2339$ &  1 &  $( 1, 0, 1)$ & $ -3.2310$ &  1 \\
        $( 0, 1, 1)$ & $ -1.8383$ &  1 &  $( 1, 1, 1)$ & $ -1.8545$ &  1 \\
        $( 0, 2, 1)$ & $ -1.7909$ &  1 &  $( 1, 2, 1)$ & $ -1.8062$ &  1 \\
        $( 0, 3, 1)$ & $ -1.7697$ &  1 &  $( 1, 3, 1)$ & $ -1.7721$ &  1 \\
        $( 0, 4, 1)$ & $  0.1605$ &  1 &  $( 1, 4, 1)$ & $  0.2381$ &  1 \\
        $( 0, 5, 1)$ & $  0.3300$ &  1 &  $( 1, 5, 1)$ & $  0.3217$ &  1 \\
        $( 0, 6, 1)$ & $  0.4068$ &  1 &  $( 1, 6, 1)$ & $  0.9628$ &  0 \\
        $( 0, 7, 1)$ & $  0.5719$ &  1 &  $( 1, 7, 1)$ & $  1.1337$ &  0 \\
        $( 0, 8, 1)$ & $  1.1680$ &  0 &  $( 1, 8, 1)$ & $  1.2303$ &  0 \\
        $( 0, 9, 1)$ & $  1.2052$ &  0 &  $( 1, 9, 1)$ & $  1.2345$ &  0 \\
        $( 0,10, 1)$ & $  2.0794$ &  0 &  $( 1,10, 1)$ & $  1.9684$ &  0 \\
        $( 0,11, 1)$ & $  2.0910$ &  0 &  $( 1,11, 1)$ & $  2.0673$ &  0 \\
        $( 0,12, 1)$ & $  2.1157$ &  0 &  $( 1,12, 1)$ & $  2.8386$ &  0 \\
        $( 0,13, 1)$ & $  2.5497$ &  0 &  $( 1,13, 1)$ & $  2.8614$ &  0 \\
        $( 0,14, 1)$ & $  2.5691$ &  0 &  $( 1,14, 1)$ & $  3.7375$ &  0 \\
        \hline
    \end{tabular}
\end{table}

